FAR: Fourier Aerial Video Recognition

We present an algorithm, Fourier Activity Recognition (FAR), for UAV video activity recognition. Our formulation uses a novel Fourier object disentanglement method to innately separate out the human agent (which is typically small) from the background. Our disentanglement technique operates in the frequency domain to characterize the extent of temporal change of spatial pixels, and exploits convolution-multiplication properties of Fourier transform to map this representation to the corresponding object-background entangled features obtained from the network. To encapsulate contextual information and long-range space-time dependencies, we present a novel Fourier Attention algorithm, which emulates the benefits of self-attention by modeling the weighted outer product in the frequency domain. Our Fourier attention formulation uses much fewer computations than self-attention. We have evaluated our approach on multiple UAV datasets including UAV Human RGB, UAV Human Night, Drone Action, and NEC Drone. We demonstrate a relative improvement of 8.02% - 38.69% in top-1 accuracy and up to 3 times faster over prior works.

==> Tables/uavhumanrgb_ablations.tex <==
\begin{table}
% \footnotesize
%\begin{subtable}{0.45\columnwidth}
\centering
\caption{\small{\textbf{Ablation experiments on UAV Human RGB.} We present ablation studies to validate the effect of FO, FA and the sampling strategy. We demonstrate that each of these individual methods (as well as their combinations) impart substantial improvement in top-1 accuracy. Cumulatively, FAR improves the baseline by $38.69\%$.}}
% \begin{center}
\resizebox{0.25\columnwidth}{!}{
\begin{tabular}{c c c c}
\toprule
FO & FA & Sampling & Top-1   \\
\midrule
\xmark & \xmark & \xmark & $21.06$ \\
\cmark & \xmark & \xmark & $25.89$ \\
\xmark & \cmark & \xmark & $24.15$ \\
\cmark & \cmark & \xmark & $27.00$ \\
\rowcolor{RowColorCode}
\cmark & \cmark & \cmark & $29.21$ \\
\bottomrule
\end{tabular}
}

\label{tab:uavhumanrgb_ablations}
\vspace{-30pt}
% \end{center}
\end{table}


==> Tables/uavhumanrgb_sota.tex <==
\begin{table}
% \footnotesize
\centering
\caption{\small{\textbf{Benchmarking UAV Human RGB and comparisons with prior art.} In experiment I, we benchmark state-of-the-art action recognition architectures at their default configurations. In experiment II, we compare with the FNet (2021), the state-of-the-art method on Fourier transform based global mixing as a replacement for self-attention. In experiment III, we benchmark FAR on various backbone architectures and configurations. We demonstrate an improvement of atleast $19.76\%$ over prior work. }}
% \begin{center}
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{c c c c c c}
\toprule
Method & Backbone & Frames & Input Size & Init. & Top-1   \\
\midrule
\multicolumn{6}{c}{I. Benchmarking UAVHuman on state-of-the-art action recognition configurations} \\
\midrule 
I3D \cite{carreira2017quo}& ResNet-101 & $8$ & $540\times960$ & Kinetics & $21.06$ \\
X3D-S \cite{feichtenhofer2020x3d}& - & $16$ & $224\times224$ & None & $21.5$ \\
X3D-M \cite{feichtenhofer2020x3d}& - & $16$ & $224\times224$ & None & $27.0$ \\
X3D-L \cite{feichtenhofer2020x3d}& - & $16$ & $224\times224$ & None & $27.6$ \\
\midrule 
\multicolumn{6}{c}{II. Comparisons with the state-of-the-art Fourier-based method} \\
\midrule 
FNet \cite{fnet} (2021) & I3D & $8$ & $540\times960$ & Kinetics & $24.39$ \\
FAR & I3D & $8$ & $540\times960$ & Kinetics & $29.21$ \\
\midrule 
\multicolumn{6}{c}{III. Results with FAR} \\
\midrule 
\rowcolor{RowColorCode}
FAR & I3D & $8$ & $540\times960$ & Kinetics & $29.21$ \\
\rowcolor{RowColorCode}
FAR & X3D-M & $8$ & $540\times540$ & None & $28.8$ \\
\rowcolor{RowColorCode}
FAR & X3D-M & $8$ & $620\times620$ & Kinetics & $39.1$ \\
\bottomrule
\end{tabular}
}

\label{tab:uavhumanrgb_sota}
\vspace{-10pt}
% \end{center}
\end{table}

